Accountability in Offline Reinforcement Learning: Explaining Decisions with a Corpus of Examples

Learning controllers with offline data in decision-making systems is an essential area of research due to its potential to reduce the risk of applications in real-world systems. However, in responsibility-sensitive settings such as healthcare, decision accountability is of paramount importance, yet has not been adequately addressed by the literature. This paper introduces the Accountable Offline Controller (AOC) that employs the offline dataset as the Decision Corpus and performs accountable control based on a tailored selection of examples, referred to as the Corpus Subset. AOC operates effectively in low-data scenarios, can be extended to the strictly offline imitation setting, and displays qualities of both conservation and adaptability. We assess AOC's performance in both simulated and real-world healthcare scenarios, emphasizing its capability to manage offline control tasks with high levels of performance while maintaining accountability.

==> tex/method_old.tex <==
\section{Preliminaries}
\paragraph{POMDP}
We develop our work under the Partially Observable Markov Decision Process (POMDP) setting, denoted as a tuple $(\mathcal{X}, \omega, \mathcal{O}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma, \rho_0)$, where $\mathcal{X} \subseteq \mathbb{R}^{d_x}$ denotes the underlying $d_x$ dimensional state space, $\omega: \mathcal{X}\mapsto \mathcal{O}$ is the emission function that maps the underlying state into a $d_o$ dimensional observation $\mathcal{O}\subseteq\mathbb{R}^{d_o}$; $\mathcal{A}\subseteq\mathbb{R}^{d_a}$ is a $d_a$ dimensional action space, transition dynamics $\mathcal{T}: \mathcal{X}\times\mathcal{A}\mapsto \mathcal{X}$ controls the underlying transition between states given actions; and the reward function $\mathcal{R}: \mathcal{X}\mapsto \mathbb{R}$ maps state into a reward scalar; we use $\gamma$ to denote the discount factor and $\rho_0$ the initial state distribution.
\paragraph{Offline Control}
Specifically, our work considers the offline learning problem: a logged dataset $\mathcal{D} = \{o^i_t, a^i_t, r^i_t, o^i_{t+1}\}^{i=1,...,N}_{t=1,...,T}$ containing $N$ trajectories with length $T$ is collected by rolling out some behavior policies in the POMDP, where $x^i_0 \sim \rho_0$ sampled from the initial state distribution and $o^i_0 =\omega(x^i_0)$, $a^i_t\sim \pi^i_b$ sampled from unknown behavior policies $\pi^i_b$. 
We denote the observational transition history until time $t$ as $h_t$, such that $h_t = (o_{<t}, a_{<t}, r_{<t}) \in \mathcal{H} \subseteq \mathbb{R}^{(d_o+d_a +1)\cdot (t-1)}$.
\paragraph{Learning Objective}
We assume the policy to be a function of observational transition history: $\pi: \mathcal{O}\times\mathcal{H}\mapsto\mathcal{A}$. The learning objective is to find a policy $\pi$ that maximizes the expected cumulative return in the POMDP:
\begin{equation}
    \max_{\pi} \mathbb{E}_{\tau \sim \rho_0,\pi,\mathcal{T}} \left[\gamma^t r_t\right]
\end{equation}
where $\tau \sim \rho_0,\pi,\mathcal{T}$ means the trajectories $\tau$ is generated by sampling initial state $x_0$ from $\rho_0$, and action $a$ from the policy $\pi$, such that:
$$\tau = \{ x_0, o_0 = \omega(x_0), a_0 = \pi(o_0, h_0=\phi), x_1 = \mathcal{T}(x_0, a_0), r_0 = \mathcal{R}(x_1), ... \}$$

\section{Accountable Control with Decision Corpus}
% We provide basic definition and motivations of the proposed method in Section~\ref{sec:method:1}, and 


\subsection{Understanding Decision-Making with a Subset of Offline Data}
\label{sec:method:1}
% To perform accountable decision-making, we build our work on the example-based explanation framework~\cite{keane2019case,crabbe2021explaining}. We introduce the \textit{Decision Corpus}, composed of a representative subset of the offline decision dataset $\mathcal{D}$. Those Decision Corpus subsets will be used to understand control time decisions. Formally, we have
In order to perform accountable decision-making, we construct our approach upon the foundation of the example-based explanation framework~\cite{keane2019case,crabbe2021explaining}. We introduce the \textit{Decision Corpus}, composed of a representative subset of the offline decision dataset $\mathcal{D}$. These Decision Corpora will be utilized for comprehending decisions made during control. Formally, this can be represented as follows:

\begin{definition}[Decision Corpus]
A \textit{Decision Corpus} $\mathcal{C}$ is defined as a subset of an offline dataset $\mathcal{D}$, indexed by $[C]:= \{1,2,...,C\}$ --- the natural numbers between $1$ and $C$. 
\begin{equation}
    \mathcal{C} = \left\{(o^c, a^c, h^c, v^c)\in\mathcal{D}\bigg|c\in [C] \right\}.
\end{equation}
\end{definition}

% In the above equation, $(o^c, a^c, h^c, v^c)\in\mathcal{D}$ denotes a transition tuple sampled from the offline dataset, and $v^c\in \mathcal{V}\subseteq \mathbb{R}$ denotes a performance measure defined according to the decision objective. e.g., $v^c$ can be defined as the ongoing cumulative return, instant reward, or risk-sensitive measure according to the user's specification.
In the equation above, the transition tuple $(o^c, a^c, h^c, v^c)\in\mathcal{D}$ is obtained from the offline dataset. The variable $v^c\in \mathcal{V}\subseteq \mathbb{R}$ represents a performance metric that is defined based on the specific decision objective. For example, $v^c$ may correspond to an ongoing cumulative return, immediate reward, or a risk-sensitive measure, as determined by the user's requirements.

Our objective is to understand the decision-making process for control time rollouts with the collected offline dataset. To do this, a naive approach is to reconstruct the control time examples with the \textit{Decision Corpus} $(o_t, a_t, h_t) = \sum_{c=1}^C w^c (o^c, a^c, h^c)$, where $w^c \in [0,1]$ and $\sum_{c=1}^C w^c = 1$. Then the corresponding performance measures $v^c$ can be used to estimate $v_t|a_t$ --- the control time return of a given decision $a_t$. 
% However, there are vital problems with this straightforward approach: 
% \begin{enumerate}[noitemsep]
%     \item The distance metric for the joint observation-action-history space is not clearly defined. Not only because different historical observations are defined over different spaces, but also because Euclidean distance can not manifest the structural information.
%     \item The transformation from the observation-action-history space to the performance measure is not necessarily a linear map: $v_t \ne \sum_{c=1}^C w^c v^c$.
% \end{enumerate}
Nonetheless, there are critical issues associated with this straightforward method:
\begin{enumerate}[noitemsep]
\item Defining a distance metric for the joint observation-action-history space presents a challenge. This is not only due to the fact that various historical observations are defined over different spaces, but also because the Euclidean distance fails to capture the structural information effectively.
\item The conversion from the observation-action-history space to the performance measure does not necessarily correspond to a linear mapping: $v_t \ne \sum_{c=1}^C w^c v^c$.
\end{enumerate}

% As an alternative solution, we propose ABC, a latent space planning algorithm that performs transparent control time control supported by \textit{Decision Corpus}.
We propose an alternative approach, Accountable Batched Controller (ABC), which is a latent space planning algorithm capable of executing accountable control, leveraging the \textit{Decision Corpus} for support.

\subsection{Linear Belief Learning for Accountable Batched Control}
To alleviate the above problems, we first introduce a specific type of belief function $\boldsymbol{b}:\mathcal{O}\times\mathcal{A}\times\mathcal{H}\mapsto\mathcal{B}\subseteq\mathbb{R}^{d_b}$, which maps a joint observation-action-history input onto a $d_b$-dimensional belief space.
\begin{property}(Linear Restricted Belief)
\label{assumption:lrb}
The performance measure function $\boldsymbol{V}: \mathcal{O}\times\mathcal{A}\times\mathcal{H}\mapsto\mathcal{V}$ can be decomposed as $\boldsymbol{V} = \boldsymbol{l} \circ \boldsymbol{b}$, where $\boldsymbol{b}:\mathcal{O}\times\mathcal{A}\times\mathcal{H}\mapsto\mathcal{B}\subseteq\mathbb{R}^{d_b}$ maps the joint observation-action-history space to a $d_b$ dimensional belief variable $b_t = \boldsymbol{b}(o_t, a_t, h_t)$ and $\boldsymbol{l}: \mathcal{B}\mapsto\mathcal{V}$ is a linear function that maps the belief $b_t$ to an output $\boldsymbol{l}(b_t)\in \mathcal{V}$. \footnote{This property can be relaxed to more general settings including when the measure function $\boldsymbol{V}$ does not exist, e.g., the strictly batched imitation learning setting. Detailed discussions can be found in Appendix~\ref{appdx:strictly_batched_il_theory}.}
\end{property}
\begin{remark}
This property is often the case with prevailing neural network approximators, where the belief state is the last activated layer before the final linear output layer. 
\end{remark}
\begin{remark}
The belief mapping function maps a $d_o + d_a + (d_o+d_a +1)\cdot (t-1)$ dimensional varied-length input into a fixed-length $d_b$ dimensional output. Usually, we have $1 = d_v < d_b \ll d_o + d_a + (d_o+d_a +1)\cdot (t-1)$. It is important to highlight that calculating the distance in the belief space is feasible, whereas it is intractable in the joint original space.
\end{remark}
Based on Property~\ref{assumption:lrb}, the linear relationship between the belief variable and the performance measure makes belief space a better choice for example-based decision understanding.
This is because decomposing the belief space breaks down the performance measure space, hence can guide action selection towards optimizing the performance metric. To be specific, we have
% as the decomposition in such a space also decomposes the performance measure space, hence can guide the action selection to maximize the performance measure. To be specific, we have
\begin{small}
\begin{equation}
\label{eqn:latent_decomposition}
    v(a_t|o_t, h_t) = \boldsymbol{l}\circ \boldsymbol{b}(o_t, a_t, h_t) = \boldsymbol{l} \circ \sum_{c=1}^C w^c \cdot \boldsymbol{b}(o^c, a^c, h^c) = \sum_{c=1}^C w^c  \cdot \boldsymbol{l} \circ \boldsymbol{b}(o^c, a^c, h^c) = \sum_{c=1}^C w^c  \cdot v^c 
\end{equation}
\end{small}
% \begin{equation}
% \begin{split}
%     v(a_t) &= \boldsymbol{l}\circ \boldsymbol{b}(o_t, a_t, h_t) \\
%     & = \boldsymbol{l} \circ \sum_{c=1}^C w_c\cdot \boldsymbol{b}(o^c, a^c, h^c) \\
%     & = \sum_{c=1}^C w_c \cdot \boldsymbol{l} \circ \boldsymbol{b}(o^c, a^c, h^c) \\
%     & = \sum_{c=1}^C w_c \cdot v^c 
% \end{split}
% \end{equation}
Although we have formally defined of the \textit{Decision Corpus}, 
% we have not explicitly specified the composition of such a subset. In the following, we introduce the principles and methods in constructing the \textit{Decision Corpus}.
its composition has not been explicitly specified. We will now present the fundamental principles and techniques employed to create a practical \textit{Decision Corpus}.
\subsection{Selection of Decision Corpus}
% Equation~(\ref{eqn:latent_decomposition}) hints that if the belief state can be decomposed as a linear combination of training-time examples, the weights used for the belief space linear decomposition can also be used to decompose and synthesize the outcome. More formally, we define the convex hull spanned by the image of decision corpus under mapping function $\boldsymbol{b}$: 
As suggested by Equation~(\ref{eqn:latent_decomposition}), if a belief state can be expressed as a linear combination of examples from the offline dataset, the same weights applied to the linear decomposition of the belief space can be utilized to decompose and synthesize the outcome. More formally, we define the convex hull spanned by the image of the decision corpus under the mapping function $\boldsymbol{b}$:
\begin{definition}(Belief Corpus)
    A \textit{Belief Corpus} $\boldsymbol{b}(\mathcal{C})$ is defined by applying the belief function $\boldsymbol{b}$ to the decision corpus $\mathcal{C}$, 
    \begin{equation}
    \boldsymbol{b}(\mathcal{C}), v = \left\{b^c = \boldsymbol{b}(o^c, a^c, h^c), v^c\bigg|(o^c, a^c, h^c, v^c)\in\mathcal{C}\right\} \subset \mathcal{B}\times\mathcal{V}
    \end{equation}
\end{definition}
\begin{definition}(Belief Corpus Hull)
    The \textit{Belief Corpus Convex Hull} spanned by a decision corpus $\mathcal{C}$ with the belief corpus $\boldsymbol{b}(\mathcal{C})$ is the convex set
    \begin{equation}
        \mathcal{C}\mathcal{B}(\mathcal{C}) = \left\{ \sum_{c=1}^C w^c b^c \bigg| w^c\in[0,1] , b^c \in \boldsymbol{b}(\mathcal{C}), \forall c\in[C], \sum_{c=1}^C w^c = 1 \right\}
    \end{equation}
\end{definition}
We note that an exact belief corpus decomposition for a control time belief value $b$ can be impossible when $b\notin \mathcal{C}\mathcal{B}(\mathcal{C})$. In such cases, the best thing we can do is to find the element $\hat{b}\in \mathcal{C}\mathcal{B}(\mathcal{C})$ that best approximates $b$. Denoting the norm in the belief space as $||\cdot||_{\mathcal{B}}$, this is equivalent to minimizing a corpus residual defined as follows:
\begin{definition}[Belief Corpus Residual]
\label{def:belief_corpus_residual}
    The \textit{Belief Corpus Residual} given a control time belief variable $b$ and a belief corpus hull $\mathcal{C}\mathcal{B}(\mathcal{C})$ is given as 
    \begin{equation}
    \label{eqn:residual}
        r_{\mathcal{C}}(b) = \min_{\tilde{b}\in \mathcal{C}\mathcal{B}(\mathcal{C})} ||b - \tilde{b}||_{\mathcal{B}}
    \end{equation}
\end{definition}
The optimizer $\hat{b} = \arg\min_{\tilde{b}\in \mathcal{C}\mathcal{B}(\mathcal{C})}||b - \tilde{b}||_{\mathcal{B}}$ can be decomposed by the belief corpus examples as $\hat{b} = \sum_{c=1}^C w^c b^c$, where the weights can be naturally interpreted as the similarity and importance in reconstructing the control time belief variable by belief corpus.
\begin{restatable}[Estimation Error Bound for $v(a_t)$]{proposition}{PROPone}
\label{prop:1}
Consider the belief variable $b_t = \boldsymbol{b}(o_t, a_t, h_t)$, the estimated value residual between $\boldsymbol{l}(b_t)$  and $\boldsymbol{l}(\hat{b})$, the optimizer of Equation~(\ref{eqn:residual}), is controlled by the corpus residual:
\begin{equation}
    ||\boldsymbol{l}(\hat{b}) - \boldsymbol{l}(b_t)||_\mathcal{V} \le ||\boldsymbol{l}||_{\mathrm{op}} \cdot r_\mathcal{C}(b_t)
\end{equation}
where $||\cdot||_\mathcal{V}$ is a norm on $\mathcal{V}$ and $||\boldsymbol{l}||_\mathrm{op} = \inf \left\{ \lambda\in\mathbb{R}^+:  ||\boldsymbol{l}(b)||_\mathcal{V} \le \lambda ||b||_\mathcal{B} \right\}$ is the operator norm for the linear mapping.
\end{restatable}
% \begin{proposition}[Estimation Error Bound for $v(a_t)$]
% \label{prop:1}
% Consider the belief variable $b_t = \boldsymbol{b}(o_t, a_t, h_t)$, the estimated value residual between $\boldsymbol{l}(b_t)$  and $\boldsymbol{l}(\hat{b})$, the optimizer of Equation~(\ref{eqn:residual}) is controlled by the corpus residual:
% \begin{equation}
%     ||\boldsymbol{l}(\hat{b}) - \boldsymbol{l}(b_t)||_\mathcal{V} \le ||\boldsymbol{l}||_{\mathrm{op}} \cdot r_\mathcal{C}(b_t)
% \end{equation}
% where $||\cdot||_\mathcal{V}$ is a norm on $\mathcal{V}$ and $||\boldsymbol{l}||_\mathrm{op} = \inf \left\{ \lambda\in\mathbb{R}^+:  ||\boldsymbol{l}(b)||_\mathcal{V} \le \lambda ||b||_\mathcal{B} \right\}$ is the operator norm for the linear mapping.
% \end{proposition}
Proposition~\ref{prop:1} indicates that minimizing the belief corpus residual also  minimizes the estimation error. 
In order to approximate the belief variables in control time accurately, we propose to use the minimum convex hull in the belief space as the decision corpus subset.
\begin{definition}[Minimal Hull]
    Denoting the decision corpora whose belief convex hull contain a belief variable $b_t$ by
    $$\mathcal{C}(b_t) = \left\{ \mathcal{C} \subseteq \mathcal{D}\bigg|b_t \in \mathcal{C}\mathcal{B}(\mathcal{C}) \right\}$$
    Among those subsets, the one that contains $d_b+1$ decision corpora and has the smallest hyper-volume forms the \textit{minimal hull}, denoted by $\tilde{\mathcal{C}}(b_t)$:
    $$
        \tilde{\mathcal{C}}(b_t):= \min_{\mathcal{C}} \int_{ \mathcal{C}\mathcal{B}(\mathcal{C})}dV
    $$
\end{definition}
\begin{restatable}[Existence and Uniqueness]{proposition}{EnU}
\label{prop:2}
Consider the belief variable $b_t = \boldsymbol{b}(o_t, a_t, h_t)$, if $r_\mathcal{C}(b_t) \le 0$ holds for $\mathcal{C} = \mathcal{D}$, then $\tilde{\mathcal{C}}(b_t)$ exists and the decomposition on this belief convex hull exists and is unique.
\end{restatable}
% \begin{proposition}[Existence and Uniqueness]
%     Consider the belief variable $b_t = \boldsymbol{b}(o_t, a_t, h_t)$, if $r_\mathcal{C}(b_t) \le 0$ holds for $\mathcal{C} = \mathcal{D}$, then $\tilde{\mathcal{C}}(b_t)$ exists and is unique.
% \end{proposition}
In this work, we use the decision corpora that construct the minimal (belief corpus convex) hull to represent the control time belief variable $b_t$. %~\footnote{DISCUSSION on scalability? (@Alihan, + Intro part )}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/teaser.png}
    \caption{We illustrate the concepts of Belief Corpus Residual and Minimal Hull in an $2$-dim example. The belief function $\boldsymbol{b}$ maps trajectories in the offline dataset (colors of \textcolor{NavyBlue}{\textbf{blue}} and \textcolor{Green}{\textbf{green}} denote that they may come from different behavior policies) onto the belief space. The \textcolor{Red}{\textbf{control trajectory}} with different sampled actions at time $t$ can also be mapped to the belief space. Some of those sampled action candidates (e.g., $a_t^{(2)}, a_t^{(3)}$) are accountable as they are surrounded by belief corpora, while in another case the corpus residual manifests the approximation error.
    }
    \label{fig:how_it_works}
\end{figure}

\subsection{Accountable Batched Control with Belief Corpus}
% According to the linear relationship between $v$ and $b$, for control time trajectory and observation $o_t, h_t$, given an action $a_t$, the corresponding estimation of performance is $\hat{v}(a_t) = \boldsymbol{l}(\hat{b}) = \sum_{c=1}^C w^c v^c$.
Consider the linear relationship between the variables $v$ and $b$, and given a specific action $a_t$, we can estimate the corresponding performance as $\hat{v}(a_t) = \boldsymbol{l}(\hat{b}) = \sum_{c=1}^C w^c v^c$, where $o_t$ and $h_t$ are the control time observation and transition history respectively.
The control action is determined by applying an arg-max operator to the action space, selecting the action with the highest estimated value that is supported by the belief corpus:
\begin{equation}
    \pi_{\mathrm{ABC}}(o_t, h_t) = \arg\max_{a_t} \hat{v}(a_t),
\end{equation}
% As we have discussed above, the exact selection of the measurement function should be determined according to the policy learning objective. In our work, we construct the value by calculating a Monte Carlo estimation of the cumulative return, as maximizing cumulative return is the most straightforward objective for batched control tasks.
As discussed earlier, the choice of measurement function $v$ depends on the objective of policy learning. In our approach, we construct $v$ using a Monte Carlo estimation of the cumulative return: $v^c=\sum_{t=t_c}^{T} \gamma^{t-t_c}r_t$, as the most straightforward choice to approach batched control tasks.


\begin{algorithm}[h!]
	\caption{Accountable Batched Control}
	\begin{algorithmic}
		\STATE \textbf{Input}
        \STATE ~~~~    Bached Dataset $\mathcal{D} = \{o^i_t, a^i_t, r^i_t, o^i_{t+1}\}^{i=1,...,N}_{t=1,...,T}$, control time observation $o_t$, control history $h_t$. Hyper-parameters: $K$ for the number of candidate actions, $\epsilon$ for the threshold.
            \STATE \textbf{Output}
        \STATE ~~~~    Accountable action $a_t$ for control.
        \STATE $\#$ 1. Optimize belief function $\boldsymbol{b}$ and linear mapping $\boldsymbol{l}$.
        \STATE ~~~~ ~~~~~~~~
        $
        \boldsymbol{b}, \boldsymbol{l}  = \arg\min_{\boldsymbol{b}, \boldsymbol{l}}\mathbb{E}_{(o^i, a^i, h^i, v^i) \in \mathcal{D}}\left(v^i - \boldsymbol{l}\circ \boldsymbol{b}(o^i, a^i, h^i)\right)^2
        $
        \STATE $\#$ 2. Sample $K$ candidate actions uniformly in the action space: $a^{k}_t\sim U(\mathcal{A}), k\in[K]$.
        \STATE $\#$ 3. Find the minimal hulls $\tilde{\mathcal{C}}(b_t)$ for each action, based on $\boldsymbol{b}$ and $b_t = \boldsymbol{b}(o_t, a^{k}_t, h_t)$.
        \STATE $\#$ 4. Minimize corpus residuals for each action candidate $a^k_t$ based on the belief corpus that spanned $\tilde{\mathcal{C}}(b_t)$.
        \STATE ~~~~ ~~~~~~~~
        $
        w^c = \arg\min_{w^c} ||\sum_{c=1}^C w^c \boldsymbol{b}(o^c, a^c, h^c) - b_t||, ~~\mathrm{s.t.}~~\sum_{c=1}^C w^c = 1, ~~(o^c, a^c, h^c) \in \tilde{\mathcal{C}}(b_t)
        $
	\STATE $\#$ 5. Estimate the value of action $a_t$ by $\hat{v}(a_t|o_t, h_t) = \sum_{c=1}^C w^c v^c$
        \STATE $\#$ 6. Outputs the candidate action that has the largest estimated value
        \STATE ~~~~~~~~~~~~
        $
        a_t = \arg\max_{a_t \in \{a^{(k)}_{t}\}} \sum_{c=1}^{C} w^c v^c, \quad
    \mathrm{s.t.}~~~r_\mathcal{C}(\boldsymbol{b}(o_t, a_t, h_t)) \le \epsilon
        $
	\end{algorithmic}
 \label{algo:1}
\end{algorithm}


\subsection{Optimization}
The optimization is conducted in a sequence: 
\begin{enumerate}
    \item optimizing the belief function and the linear mapping in predicting given performance measure: 
    $$
    \boldsymbol{b}, \boldsymbol{l}  = \arg\min_{\boldsymbol{b}, \boldsymbol{l}}\mathbb{E}_{(o^i, a^i, h^i, v^i) \in \mathcal{D}}\left(v^i - \boldsymbol{l}\circ \boldsymbol{b}(o^i, a^i, h^i)\right)^2
    $$
    where $\boldsymbol{l}$ is limited to be a linear function and $\boldsymbol{b}$ the belief mapping.
    \item during control time roll-out, given observation $o_t$ and historical input $h_t$, and an action proposal $a_t$, reconstruct the belief $b_t = \boldsymbol{b}(o_t, a_t, h_t)$ with the minimal hull $\tilde{\mathcal{C}}(b_t)$ by minimizing the \textit{Belief Corpus Residual}, such that
    $$
    w^c = \arg\min_{w^c} ||\sum_{c=1}^C w^c \boldsymbol{b}(o^c, a^c, h^c) - b_t||, ~~\mathrm{s.t.}~~\sum_{c=1}^C w^c = 1, ~~(o^c, a^c, h^c) \in \tilde{\mathcal{C}}(b_t)
    $$
    And estimate the value of action $a_t$ by $\hat{v}(a_t|o_t, h_t) = \sum_{c=1}^C w^c v^c$
    \item We perform a sampling-based optimization on the action space while taking the corpus residual into consideration. To be specific, we first uniformly sample $K$ actions in the action space at each time step, $\{a^{(k)}_{t}\} \sim U(\mathcal{A})$. We then search for the action that corresponds to the maximal performance measure, while constraining the belief corpus residual to be smaller than a certain threshold $\epsilon\ge0$: 
\begin{equation}
\label{eqn:residual_opt}
    \pi_{\mathrm{ABC}}(o_t, h_t) = \arg\max_{a_t \in \{a^{(k)}_{t}\}} \sum_{c=1}^{C} w^c v^c, \quad
    \mathrm{s.t.}~~~r_\mathcal{C}(\boldsymbol{b}(o_t, a_t, h_t)) \le \epsilon
\end{equation}
\end{enumerate}
Pseudo-code is provided in Algorithm~\ref{algo:1}.% in Appendix~\ref{appdx:algo:1}.















